Topology-Preserving Off-screen Visualization: Effects of Projection Strategy and Intrusion Adaption

With the increasing amount of data being visualized in large information spaces, methods providing data-driven context have become indispensable. Off-screen visualization techniques, therefore, have been extensively researched for their ability to overcome the inherent trade-off between overview and detail. The general idea is to project off-screen located objects back to the available screen real estate. Detached visual cues, such as halos or arrows, encode information on position and distance, but fall short showing the topology of off-screen objects. For that reason, state of the art techniques integrate visual cues into a dedicated border region. As yet, the dimensions of the navigated space are not reflected properly, which is why we propose to adapt the intrusion of the border pursuant to the position in space. Moreover, off-screen objects are projected to the border region using one out of two projection methods: Radial or Orthographic. We describe a controlled experiment to investigate the effect of the adaptive border intrusion to the topology as well as the users' intuition regarding the projection strategy. The results of our experiment suggest to use the orthographic projection strategy for unconnected point data in an adaptive border design. We further discuss the results including the given informal feedback of participants.

==> rw_table_tr.tex <==
%!TEX root = ../paper.tex
% !TeX encoding = UTF-8
% !TeX spellcheck = en_US
%{
%\scriptsize
%\renewcommand{\arraystretch}{1.5}
\setlength\extrarowheight{2pt}
\begin{tabular}{| p{2.3cm} | c | c | c | c | p{1.9cm} |}
	
	\hline
	
	\textbf{Paper} & \textbf{Direction} & \textbf{Distance} & \textbf{Topology} & \textbf{Border} & \textbf{Projection} \\
	
	\hline \hline
    
    %& & & & & \\ \hline
    
    City Lights \cite{DBLP:conf/chi/ZellwegerMGSB03} & \pie{360} & \pie{180} &  &  & orthographic, radial \\ \hline
    
    Halo \cite{DBLP:conf/chi/BaudischR03} & \pie{360} & \pie{360} & & & (orthographic) \\ \hline
    
    Hopping \cite{DBLP:conf/chi/IraniGY06} & \pie{360} & \pie{360} & \pie{180} & & orthographic, radial \\ \hline
    
    EdgeRadar \cite{DBLP:conf/chi/GustafsonI07} & \pie{360} & \pie{360} & \pie{360} & \ding{51} & orthographic \\ \hline
    
    Wedge \cite{DBLP:conf/chi/GustafsonBGI08} & \pie{360} & \pie{360} & & & orthographic (adapted) \\ \hline
    
    Predictive Jumping \cite{DBLP:conf/apchi/TakashimaSTKK08} & \pie{360} & \pie{360} & & & orthographic \\ \hline
    
    HaloDot \cite{gonccalves2011halodot} & \pie{360} & \pie{180} & & & (orthographic) \\ \hline
    
    EdgeSplit \cite{DBLP:conf/mhci/HossainHLI12} & \pie{360} & \pie{360} & \pie{360} & \ding{51} & orthographic \\ \hline
    
    Off-screen data on tablets \cite{games2013visualization} & \pie{360} & \pie{360} & & \ding{51} & orthographic, radial \\ \hline
    
    Sparkle \cite{DBLP:conf/nordichi/MullerLHB14} & \pie{360} & \pie{360} & & & orthographic \\ \hline
    
    Uncertainty Visualization \cite{eurova.20151103} & \pie{360} & \pie{180} & \pie{360} & \ding{51} & radial \\ \hline
    
    Ambient Grids \cite{eurovisshort.20151125} & \pie{360} & \pie{180} & \pie{360} & \ding{51} & orthographic \\ \hline
    
    Glowworms and Fireflies \cite{DBLP:conf/chi/PertenederGLSH16} & \pie{360} & \pie{360} & & & orthographic \\ \hline
    
    \hline
\end{tabular}%} %\quad}
